Learned Full Waveform Inversion Incorporating Task Information for Ultrasound Computed Tomography

Ultrasound computed tomography (USCT) is an emerging imaging modality that holds great promise for breast imaging. Full-waveform inversion (FWI)-based image reconstruction methods incorporate accurate wave physics to produce high spatial resolution quantitative images of speed of sound or other acoustic properties of the breast tissues from USCT measurement data. However, the high computational cost of FWI reconstruction represents a significant burden for its widespread application in a clinical setting. The research reported here investigates the use of a convolutional neural network (CNN) to learn a mapping from USCT waveform data to speed of sound estimates. The CNN was trained using a supervised approach with a task-informed loss function aiming at preserving features of the image that are relevant to the detection of lesions. A large set of anatomically and physiologically realistic numerical breast phantoms (NBPs) and corresponding simulated USCT measurements was employed during training. Once trained, the CNN can perform real-time FWI image reconstruction from USCT waveform data. The performance of the proposed method was assessed and compared against FWI using a hold-out sample of 41 NBPs and corresponding USCT data. Accuracy was measured using relative mean square error (RMSE), structural self-similarity index measure (SSIM), and lesion detection performance (DICE score). This numerical experiment demonstrates that a supervised learning model can achieve accuracy comparable to FWI in terms of RMSE and SSIM, and better performance in terms of task performance, while significantly reducing computational time.

==> fista_alg.tex <==
\begin{algorithm2e}
\SetAlgoLined

Let $X_{j}$ be points centered at each pixel for time $k_j$ and $A$ be the static imaging operator.\\

Initialize neural field $\Phi_\xi$. \\ 
Initialize Fista object $\Psi = \operatorname{Copy}(\Phi_\xi)$.\\
Initialize $t = 1$.


 \While{While convergence criterion is not met}{
 Set $\Phi_{old} = \operatorname{Copy}(\Phi_\xi)$ \\ 
 $t^{old} \leftarrow t$\\
 $ t \leftarrow \frac{1+\sqrt{1+4t^2}}{2}$\\
 
 Randomly select collection of frames $\{k_1,\hdots, k_F\}$ with view projection operators $\{P_1,\hdots, P_F\}$, where measurements at frame $k_j$ correspond to $P_j\Phi_\xi(X_{j})$ \\ 
 
 Declare gradient object
 
 $$G_j:= \frac{1}{\sigma^2} A^TP_j^T(P_jA\Psi(X_{k_j}) - m_j)$$
 
 Set global stepsize 
 
 $$\alpha = \sigma^2 \frac{\sum_{j=1}^FG_j^TG_j}{\sum_{j=1}^F G^T_jA^TP_j^TP_jAG_j}$$\\ 

 $\Phi_\xi \leftarrow \operatorname{Prox}_{\alpha, \Reg}^\xi(\Psi - \alpha G)$ or equivalently $$\xi \leftarrow \argmin_\xi \frac{1}{2\alpha} \|\Phi_\xi - \Psi +\alpha G\|^2 + \Reg(\Phi_{\xi})$$
 
 $$c := \frac{t^{old} - 1}{t}$$\\
 
 $\Psi \leftarrow \operatorname{Sum}((1+c)\operatorname{Copy}(\Phi_\xi), -c\operatorname{Copy}(\Phi_{old}))$

 
 
 
 }
 

 \caption{Neural Field Stochastic Fista}
\end{algorithm2e}

==> math_notations.tex <==
\section{Mathematical Notation}
Table \ref{tab:notation} summarizes the mathematical notations and symbols used in this work.


    \label{tab:notation}
\begin{table}[H]
    \centering
    \caption{Table of mathematical notations and symbols}
    \begin{tabular}{c|l}
        $\ipar \in \mathbb{U}$ & Infinite dimensional image  \\
        $\data \in \D$ & Finite dimensional measurements \\ 
        $\H:\mathbb{U} \rightarrow \D$ & Continuous-to-discrete imaging operator\\
        $\mathbf{H}:\R^{NK} \rightarrow \D$& Discrete-to-discrete imaging operator\\
        $\noise \in \D$ & Additive noise in measurement space \\ 
        $\sigma\in \R$ & Standard deviation of white Gaussian noise \\ 
        $x \in \Omega$ & Spatial coordinates for image \\ 
        $t \in [0,T]$ & Time coordinates for image\\
        $\Omega_T = \Omega \times [0,T]$ & Domain over which image coordinates are defined \\ 
        $\LI:\mathbb{U}\rightarrow \R$ & Continuous data fidelity functional \\
        $\mathbf{L}:\R^{NK} \rightarrow \R$& Discrete data fidelity function \\
        $\Reg: \mathbb{U}\rightarrow \R$ & Regularization functional \\ 
        $\mathbf{R}:\R^{NK} \rightarrow \R$& Discrete regularization function\\
        $\J = \LI + \Reg$ & Continuous cost functional\\
        $\mathbf{J} = \mathbf{L} + \mathbf{R}$& Discrete cost function\\
        $N$ & Number of pixels \\ 
        $K$ & Number of frames \\ 
        $\boldsymbol{\ipar } \in \R^{NK}$ & discrete representation of $\ipar$ \\
        $\{\beta_n:\Omega \rightarrow \R\}_{n=1}^N$ & basis for discrete representation. \\ 
        $\alpha \in \R^{K*N}$ & spanning coefficients for discrete representation \\ 
        $D_\nabla$ & finite difference gradient operator \\ 
        $TV_D$ & Discrete total variation using finite-differences\\
        $TV_S$ & Stochastic total variation using automatic differentiation \\ 
        $\boldsymbol{F} \in \R^{N \times K}$ & matrix representation of spanning coefficients \\ 
        $\operatorname{Nuc}:\R^{N\times K} \rightarrow \R$ & Nuclear norm functional\\
        $\gamma > 0$ & regularization weight\\ 
        $\xi \in \R^W$ & Neural Network weights\\
        $\Phi_\xi : \Omega_T \rightarrow \R$ & Neural field with weights $\xi$\\
        $P$ & Number of partitions\\
        $\Psi = (\psi^1,\hdots \psi^P)^T$ & Partition of unity \\ 
        $M$ & Number of basis functions \\ 
        $B = (b_1,\hdots , b_M)^T$ &Spanning functions \\ 
        $C \in \R^{P \times M}$ & Coefficient matrix \\ 
        $\ipar^{\Psi,B}_C = \Psi^TCB:$ & POU defined function \\ 
        $\eta$ & Weights of Partition of unity network \\ 
        $\Psi_\eta :\Omega_T \rightarrow \R^P$ & POU parametrized by neural network \\ 
        $\Phi_{(\eta,B)} = f^{\Psi_\eta,B}_C$& POUnet \\
        $\rho > 0$ & Training weight to enforce distribution of partitions\\
        $\tau >0$ & Training weight to promote sparsity of distributions \\
        $\epsilon >0$ & Perturbing term to prevent singularities \\
        $\crt$& Stationary CRT \\ 
        $\crt_D$ & Dynamic CRT \\ 
        
        
    \end{tabular}
\end{table}
